Anvil: An integration of artificial intelligence, sampling techniques, and a combined CAD-CFD tool

In this work, we introduce an open-source integrated CAD-CFD tool, Anvil, which combines FreeCAD for CAD modeling and OpenFOAM for CFD analysis, along with an AI-based optimization method (Bayesian optimization) and other sampling algorithms. Anvil serves as a scientific machine learning tool for shape optimization in three modes: data generation, CFD evaluation, and shape optimization. In data generation mode, it automatically runs CFD evaluations and generates data for training a surrogate model. In optimization mode, it searches for the optimal design under given requirements and optimization metrics. In CFD mode, a single CAD file can be evaluated with a single OpenFOAM run. To use Anvil, experimenters provide a JSON configuration file and a parametric CAD seed design. Anvil can be used to study solid-fluid dynamics for any subsonic flow conditions and has been demonstrated in various simulation and optimization use cases. The open-source code for the tool, installation process, artifacts (such as CAD seed designs and example STL models), experimentation results, and detailed documentation can be found at \url{https://github.com/symbench/Anvil}.

==> t00Authors.tex <==
\author{Harsh Vardhan }
\email{harsh.vardhan@vanderbilt.edu}
\orcid{0000-0001-8273-2931}

\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}

\author{Umesh Timalsina}
\email{umesh.timalsina@vanderbilt.edu}
\orcid{0000-0002-5430-3993}



\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}

\author{Michael Sandborn}
\email{michael.sandborn@vanderbilt.edu}
\orcid{0000-0001-8592-6758}



\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}

\author{David Hyde}
\email{david.hyde.1@vanderbilt.edu}
\orcid{0009-0004-4950-5533}



\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}
\renewcommand{\shortauthors}{}


\author{Peter Volgyesi}
\email{peter.volgyesi@vanderbilt.edu}
\orcid{0000-0002-7478-4317}



\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}
\renewcommand{\shortauthors}{}

\author{Janos Sztipanovits}
\email{janos.sztipanovits@vanderbilt.edu}
\orcid{0000-0002-8360-6299}



\affiliation{%
  \institution{Vanderbilt University}
  \city{Nashville}
  \state{TN}
  \country{USA}
}
\renewcommand{\shortauthors}{}

